WHAM: Reconstructing World-grounded Humans with Accurate 3D Motion

The estimation of 3D human motion from video has progressed rapidly but current methods still have several key limitations. First, most methods estimate the human in camera coordinates. Second, prior work on estimating humans in global coordinates often assumes a flat ground plane and produces foot sliding. Third, the most accurate methods rely on computationally expensive optimization pipelines, limiting their use to offline applications. Finally, existing video-based methods are surprisingly less accurate than single-frame methods. We address these limitations with WHAM (World-grounded Humans with Accurate Motion), which accurately and efficiently reconstructs 3D human motion in a global coordinate system from video. WHAM learns to lift 2D keypoint sequences to 3D using motion capture data and fuses this with video features, integrating motion context and visual information. WHAM exploits camera angular velocity estimated from a SLAM method together with human motion to estimate the body's global trajectory. We combine this with a contact-aware trajectory refinement method that lets WHAM capture human motion in diverse conditions, such as climbing stairs. WHAM outperforms all existing 3D human motion recovery methods across multiple in-the-wild benchmarks. Code will be available for research purposes at http://wham.is.tue.mpg.de/

==> tables/finals/Table1.tex <==
\newcolumntype{?}{!{\vrule width 0.75pt}}

\begin{table*}[tbh]
\centering
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.8\textwidth}{!}
{\small{
\begin{tabular}{cl?cccc?cccc?cccc}
\cmidrule[0.75pt]{1-14}
& & \multicolumn{4}{c}{3DPW (14)} & \multicolumn{4}{c}{RICH (24)} & \multicolumn{4}{c}{EMDB (24)} \\
% \cmidrule(lr){3-13}
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}

& Models & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} \\
\cmidrule{1-14}

\multirow{6}{1em}{\rotatebox[origin=c]{90}{per-frame}} 
& SPIN \cite{spin} & 59.2 & 96.9 & 112.8 & 31.4 & 69.7 & 122.9 & 144.2 & 35.2 & 87.1 & 140.7 & 166.1 & 41.3 \\

& CLIFF$^*$ \cite{cliff} & 43.0 & 69.0 & 81.2 & 22.5 & 56.6 & 102.6 & 115.0 & 22.4 & 68.3 & 103.5 & 123.7 & 24.5 \\

& HMR2.0 \cite{hmr2.0} & 44.4 & 69.8 & 82.2 & 18.1 & 48.1 & 96.0 & 110.9 & 18.8 & 60.7 & 98.3 & 120.8 & 19.9 \\

& BEDLAM-CLIFF$^*$ \cite{bedlam} & 43.0 & 66.9 & 78.5 & 31.0 & 50.2 & 84.4 & 95.6 & 29.3 & 60.9 & 98.2 & 111.6 & 36.1 \\

& ReFit$^*$ \cite{refit} & 40.5 & 65.3 & 75.1 & 18.5 & 47.9 & 80.7 & 92.9 & 17.1 & 58.6 & 88.0 & 104.5 & 20.7 \\

& ReFit-B$^*$ \cite{refit} & 38.2 & 57.6 & \textbf{67.6} & 21.4 & 44.5 & \textbf{77.1} & \textbf{87.8} & 18.3 & 57.1 & 91.0 & 105.7 & 23.1 \\

\cmidrule{1-14}

\multirow{12}{1em}{\rotatebox[origin=c]{90}{temporal}} 
& PACE \cite{pace} & -- & -- & -- & -- & 49.3 & --  & -- & 8.8 & -- & -- & -- & -- \\

& TCMR$^*$ \cite{tcmr} & 52.7 & 86.5 & 101.4 & 6.0 & 65.6 & 119.1 & 137.7 &  5.0 & 79.8 & 127.7 & 150.2 & 5.3 \\

& VIBE$^*$ \cite{vibe} & 51.9 & 82.9 & 98.4 & 18.5 & 68.4 & 120.5 & 140.2 & 21.8 & 81.6 & 126.1 & 149.9 & 26.5 \\

& MPS-Net$^*$ \cite{mpsnet}  & 52.1 & 84.3 & 99.0 & 6.5 & 67.1 & 118.2 & 136.7 & 5.8 & 81.4 & 123.3 & 143.9 & 6.2 \\

& GLoT$^*$ \cite{glot} & 50.6 & 80.7 & 96.4 & \textbf{6.0} & 65.6 & 114.3 & 132.7 & 5.2 & 79.1 & 119.9 & 140.8 & 5.4 \\

& GLAMR \cite{glamr} & 51.1 & -- & -- & 8.0 & 79.9 & -- & -- & 107.7 & 73.8 & 113.8 & 134.9 & 33.0 \\

& TRACE$^*$ \cite{trace} & 50.9 & 79.1 & 95.4 & 28.6 & -- & -- & -- & -- & 71.5 & 110.0 & 129.6 & 25.5 \\

& SLAHMR \cite{slahmr} & 55.9& -- & -- & -- & 52.5 & -- & -- & 9.4 & 69.7 & 93.7 & 111.3 & 7.1 \\

\cmidrule{2-14}
& \textbf{WHAM (Res)}$^*$  & 40.2 & 62.7 & 75.1 & 6.3 & 51.8 & 89.5 & 103.2 & \textbf{5.0} & 57.8 & 84.0 & 99.7 & \textbf{5.2} \\
& \textbf{WHAM (HR)}$^*$  & 39.0 & 62.6 & 74.8 & 6.4 & 49.1 & 84.6 & 96.4 & 5.2 & 57.1 & 85.7 & 103.2 & 5.6 \\
&\textbf{WHAM (ViT)}$^*$ & 36.2 & 58.6 & 70.4 & 6.6 & 44.7 & 79.7 & 90.5 & 5.4 & 50.7 & 78.9 & 93.2 & 5.4 \\
&\textbf{WHAM-B (ViT)}$^*$ & \textbf{35.4} & \textbf{57.3} & 68.0 & 6.9 & \textbf{43.4} & 79.6 & 90.2 & 5.3 & \textbf{47.8} & \textbf{78.2} & \textbf{90.8} & 5.4 \\

\cmidrule[0.75pt]{1-14}
\end{tabular}
}}
    \vspace{-0.075in}
\caption{Quantitative comparison of state-of-the-art models on the 3DPW \cite{3dpw}, RICH \cite{rich}, and EMDB \cite{emdb} datasets. 
Ordering of per-frame and temporal methods is done separately by descending MPJPE on EMDB. For testing on EMDB, we follow the protocol of \textit{EMDB 1} \cite{emdb}. Parenthesis denotes the number of body joints used to compute MPJPE and PA-MPJPE, and $^*$ denotes models trained with the 3DPW training set.
Bold numbers denote the most accurate method in each column. Accel is in $m/s^2$, all other errors are in $mm$.
}
\label{tab:table1}
\end{table*}

==> tables/tableX_ablation.tex <==
\newcolumntype{?}{!{\vrule width 0.95pt}}

%\begin{center}
    \begin{table}
    \centering
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.99\columnwidth}{!}{{\small{
    \begin{tabular}{l?cccccc}
    \cmidrule{1-7}
    & \multicolumn{6}{c}{EMDB 2} \\
    \cmidrule(lr){2-7}
    
    Methods & PA-MPJPE & PVE & RTE & ROE & ERVE & EFVE \\
    \cmidrule{1-7}
    % w/o $F_I$ & 44.1 & 84.9 & 8.8 & 40.6 & 15.1 & 20.7 \\
    % w/o lifting & 108.9 & 187.5 & 18.6 & 98.3 & 29.4 & 36.8\\
    % w/o traj. ref. & 41.9 & 74.7 & 8.8 & 40.2 & 14.4 & 20.9 \\
    % w/o $\omega$ & 40.7 & 74.5 & 18.3 & 77.1 & 14.4 & 20.8 \\
    % WHAM (Ours) & 41.9 & 74.7 & 8.6 & 40.2 & 14.8 & 19.8 \\
    w/o $F_I$ & 44.1 & 84.9 & 9.4 & 41.6 & 15.1 & 20.7 \\
    w/o lifting & 108.9 & 187.5 & 18.5 & 98.3 & 29.4 & 36.8\\
    w/o traj. ref. & 41.9 & 74.7 & 9.0 & 40.4 & 14.4 & 20.9 \\
    w/o $\omega$ & 40.7 & 74.5 & 18.3 & 77.1 & 14.4 & 20.8 \\
    WHAM (Ours) & 41.9 & 74.7 & 8.8 & 40.4 & 14.8 & 19.8 \\
    \cmidrule{1-7}
    \end{tabular}
    }}}
    \vspace{-0.075in}
    \caption{Ablation experiments. See text.}
    \label{tab:ablation}
    \end{table}
%\end{center}


==> tables/tableX_neural_init.tex <==
\newcolumntype{?}{!{\vrule width 0.5pt}}

\begin{center}
    \begin{table}
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.48\textwidth}{!}{{\small{
    \begin{tabular}{l?cccc}
    \cmidrule{1-5}
    & \multicolumn{4}{c}{3DPW} \\
    \cmidrule(lr){2-5}
    
    Methods & PA-MPJPE & MPJPE & PVE & Accel \\
    \cmidrule{1-5}
    w/o Neural State Initialization & \textbf{37.8} & 64.5 & 76.3 & 6.9 \\
    \textbf{WHAM} & \textbf{37.8} & \textbf{60.8} & \textbf{72.5} & \textbf{6.8} \\
    \cmidrule{1-5}
    \end{tabular}
    }}}
    \caption{Quantitative analysis of neural state initialization on the 3DPW \cite{3dpw} dataset.}
    \label{tab:neural_init}
    \end{table}
\end{center}


==> tables/tableX_quant.tex <==
\newcolumntype{?}{!{\vrule width 0.75pt}}

\begin{table*}[tbh]
\centering
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.8\textwidth}{!}
{\small{
\begin{tabular}{cl?cccc?cccc?cccc}
\cmidrule[0.75pt]{1-14}
& & \multicolumn{4}{c}{3DPW (14)} & \multicolumn{4}{c}{RICH (24)} & \multicolumn{4}{c}{EMDB (24)} \\
% \cmidrule(lr){3-13}
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}

& Models & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} \\
\cmidrule{1-14}

\multirow{6}{1em}{\rotatebox[origin=c]{90}{per-frame}} 
% & SPIN \cite{spin} & 59.2 & 96.9 & 116.4 & 34.9 & 69.7 & 122.9 & 144.2 & 39.1 & 87.1 & 140.3 & 174.9 & 45.9 \\

% & PARE$^*$ \cite{pare} & 46.5 & 74.5 & 88.6 & -- & 60.7 & 109.2 & 123.5 & -- & 72.2 & 113.9 & 133.2 & -- \\

% & CLIFF$^*$ \cite{cliff} & 43.0 & 69.0 & 81.2 & 25.0 & 56.6 & 102.6 & 115.0 & 24.8 & 68.1 & 103.3 & 128.0 & 27.2 \\

% & HybrIK$^*$ \cite{hybrik} & 41.8 & 71.6 &  82.3 & -- & 56.4 & 96.8 & 110.4 & -- & 65.6 & 103.0 & 122.2 & -- \\

% & HMR2.0 \cite{hmr2.0} & 44.4 & 69.8 & 84.0 & 20.1 & 48.1 & 96.0 & 110.9 & 20.9 & 60.6 & 98.0 & 120.3 & 22.0 \\

% & BEDLAM-CLIFF$^*$ \cite{bedlam} & 43.0 & 66.9 & 78.5 & 34.4 & 50.2 & 84.4 & 95.6 & 32.6 & 60.6 & 98.0 & 111.6 & 40.1 \\

% \cmidrule{1-14}

% \multirow{12}{1em}{\rotatebox[origin=c]{90}{temporal}} 
% & PACE \cite{pace} & -- & -- & -- & -- & 49.3 & --  & -- & 8.8 & -- & -- & -- & -- \\
% & TCMR$^*$ \cite{tcmr} & 52.7 & 86.5 & 102.9 & 6.7 & 65.6 & 119.1 & 137.7 &  \textbf{5.6} & 79.6 & 127.6 & 147.9 & \textbf{5.8} \\

% & VIBE$^*$ \cite{vibe} & 51.9 & 82.9 & 99.1 & 20.6 & 68.4 & 120.5 & 140.2 & 24.3 & 81.4 & 125.9 & 146.8 & 29.5 \\
% & MPS-Net$^*$ \cite{mpsnet}  & 52.1 & 84.3 & 99.7 & 7.3 & 67.1 & 118.2 & 136.7 & 6.4 & 81.3 & 123.1 & 138.4 & 6.9 \\

% & GLoT$^*$ \cite{glot} & 50.6 & 80.7 & 96.3 & \textbf{6.6} & 65.6 & 114.3 & 132.7 & 5.8 & 78.8 & 119.7 & 138.4 & 6.0 \\

% & GLAMR \cite{glamr} & 51.1 & -- & -- & 8.9 & 79.9 & -- & -- & 107.7 & 73.5 & 113.6 & 133.4 & 36.6 \\

% & TRACE$^*$ \cite{trace} & 50.9 & 79.1 & 97.3 & 31.7 & -- & -- & -- & -- & 70.9 & 109.9 & 127.4 & 28.2 \\

% & SLAHMR \cite{slahmr} & 55.9& -- & -- & -- & 52.5 & -- & -- & 9.4 & 69.5 & 93.5 & 110.7 & 7.9 \\

% % & MAED$^*$ \cite{maed} & 45.7 & 79.1 & 92.6 & 17.6 & -- & -- & -- & & -- & -- & -- & -- \\

% \cmidrule{2-14}
% & \textbf{WHAM (Res)}$^*$  & 41.7 & 65.7 & 79.8 & 7.5 & 53.1 & 91.4 & 105.6 & 5.9 & 58.9 & 90.3 & 105.7 & 6.3 \\
% & \textbf{WHAM (HR)}$^*$  & 40.9 & 64.5 & 78.8 & 7.6 & 50.7 & 88.0 & 100.8 & 6.9 & 56.8 & 88.8 & 105.7 & 6.5 \\
% &\textbf{WHAM (ViT)}$^*$ & 38.3 & 60.5 & 73.8 & 7.6 & 46.2 & 84.1 & 95.5 & 6.1 & 52.2 & 85.5 & 101.0 & 6.8 \\
% &\textbf{WHAM-B (ViT)}$^*$ & \textbf{37.3} & \textbf{59.2} & \textbf{71.7} & 7.6 & \textbf{44.7} & \textbf{82.6} & \textbf{93.2} & 6.2 & \textbf{49.4} & \textbf{81.5} & \textbf{94.3} & 6.5 \\

& SPIN \cite{spin} & 59.2 & 96.9 & 112.8 & 31.4 & 69.7 & 122.9 & 144.2 & 35.2 & 87.1 & 140.3 & 174.9 & 41.3 \\

& PARE$^*$ \cite{pare} & 46.5 & 74.5 & 88.6 & -- & 60.7 & 109.2 & 123.5 & -- & 72.2 & 113.9 & 133.2 & -- \\

& CLIFF$^*$ \cite{cliff} & 43.0 & 69.0 & 81.2 & 22.5 & 56.6 & 102.6 & 115.0 & 22.4 & 68.1 & 103.3 & 128.0 & 24.5 \\

& HybrIK$^*$ \cite{hybrik} & 41.8 & 71.6 &  82.3 & -- & 56.4 & 96.8 & 110.4 & -- & 65.6 & 103.0 & 122.2 & -- \\

& HMR2.0 \cite{hmr2.0} & 44.4 & 69.8 & 82.2 & 18.1 & 48.1 & 96.0 & 110.9 & 18.8 & 60.6 & 98.0 & 120.3 & 19.8 \\

& BEDLAM-CLIFF$^*$ \cite{bedlam} & 43.0 & 66.9 & 78.5 & 31.0 & 50.2 & 84.4 & 95.6 & 29.3 & 60.6 & 98.0 & 111.6 & 36.1 \\
\cmidrule{1-14}

\multirow{12}{1em}{\rotatebox[origin=c]{90}{temporal}} 
& PACE \cite{pace} & -- & -- & -- & -- & 49.3 & --  & -- & 8.8 & -- & -- & -- & -- \\

& TCMR$^*$ \cite{tcmr} & 52.7 & 86.5 & 101.4 & 6.0 & 65.6 & 119.1 & 137.7 &  \textbf{5.0} & 79.6 & 127.6 & 147.9 & \textbf{5.3} \\

& VIBE$^*$ \cite{vibe} & 51.9 & 82.9 & 98.4 & 18.5 & 68.4 & 120.5 & 140.2 & 21.8 & 81.4 & 125.9 & 146.8 & 26.6 \\

& MPS-Net$^*$ \cite{mpsnet}  & 52.1 & 84.3 & 99.0 & 6.5 & 67.1 & 118.2 & 136.7 & 5.8 & 81.3 & 123.1 & 138.4 & 6.2 \\

& GLoT$^*$ \cite{glot} & 50.6 & 80.7 & 96.4 & \textbf{6.0} & 65.6 & 114.3 & 132.7 & 5.2 & 78.8 & 119.7 & 138.4 & 5.4 \\

& GLAMR \cite{glamr} & 51.1 & -- & -- & 8.0 & 79.9 & -- & -- & 107.7 & 73.5 & 113.6 & 133.4 & 32.9 \\

& TRACE$^*$ \cite{trace} & 50.9 & 79.1 & 95.4 & 28.6 & -- & -- & -- & -- & 70.9 & 109.9 & 127.4 & 25.5 \\

& SLAHMR \cite{slahmr} & 55.9& -- & -- & -- & 52.5 & -- & -- & 9.4 & 69.5 & 93.5 & 110.7 & 7.1 \\

% & MAED$^*$ \cite{maed} & 45.7 & 79.1 & 92.6 & 17.6 & -- & -- & -- & & -- & -- & -- & -- \\

\cmidrule{2-14}
& \textbf{WHAM (Res)}$^*$  & 41.7 & 65.7 & 78.7 & 6.6 & 53.1 & 91.4 & 105.6 & 5.3 & 58.9 & 90.3 & 106.1 & 5.7 \\
& \textbf{WHAM (HR)}$^*$  & 40.9 & 64.5 & 77.7 & 6.8 & 50.7 & 88.0 & 100.8 & 5.7 & 58.4 & 89.5 & 107.7 & 6.5 \\
&\textbf{WHAM (ViT)}$^*$ & 37.8 & 60.8 & 72.5 & 6.8 & 46.2 & 84.1 & 95.5 & 5.5 & 53.4 & 87.3 & 102.9 & 5.7 \\
&\textbf{WHAM-B (ViT)}$^*$ & \textbf{37.2} & \textbf{59.4} & \textbf{71.0} & 6.9 & \textbf{44.7} & \textbf{82.6} & \textbf{93.2} & 5.6 & \textbf{48.8} & \textbf{80.7} & \textbf{93.7} & 5.9 \\

\cmidrule[0.75pt]{1-14}
\end{tabular}
}}
    \vspace{-0.075in}
\caption{Quantitative comparison of state-of-the-art models on the 3DPW \cite{3dpw}, RICH \cite{rich}, and EMDB \cite{emdb} datasets. 
Ordering of per-frame and temporal methods is done separately by descending MPJPE on EMDB. For testing on EMDB, we follow the protocol of \textit{EMDB 1} \cite{emdb}. Parenthesis denotes the number of body joints used to compute MPJPE and PA-MPJPE, and $^*$ denotes models trained with the 3DPW training set.
Bold numbers denote the most accurate method in each column. Accel is in $m/s^2$, all other errors are in $mm$.
}
\label{tab:quant_hps}
\end{table*}

==> tables/tableX_quant_cam.tex <==
\newcolumntype{?}{!{\vrule width 0.95pt}}

\begin{center}
    \begin{table}
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.4\textwidth}{!}{{\small{
    \begin{tabular}{l?cc}
    \cmidrule{1-3}
    & \multicolumn{2}{c}{EMDB Set 2} \\
    \cmidrule(lr){2-3}
    
    Models & Orientation & Translation \\
    \cmidrule{1-3}
    
    GLAMR \cite{glamr} & 70.6 & 7.4\\
    TRACE \cite{trace} & 69.6 & 8.8\\
    DPVO \cite{dpvo} & 42.6 & 7.5\\
    
    \cmidrule{1-3}
    \textbf{WHAM (w. DPVO)} & 35.4 & 3.9\\
    \textbf{WHAM (w. GT)} & \textbf{23.7} & \textbf{3.5} \\
    \cmidrule{1-3}
    \end{tabular}
    }}}
    \caption{Quantitative comparison in camera trajectory recovery on EMDB \cite{emdb} dataset.}
    \label{tab:quant_cam}
    \end{table}
\end{center}


==> tables/tableX_quant_global.tex <==
\newcolumntype{?}{!{\vrule width 0.95pt}}

\begin{center}
    \begin{table}
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.99\columnwidth}{!}{{\small{
    \begin{tabular}{l?cccccc}
    \cmidrule{1-7}
    & \multicolumn{6}{c}{EMDB Set 2} \\
    \cmidrule(lr){2-7}
    
    Models & ROE & RTE & ERVE & EFVE & COE & CTE \\
    \cmidrule{1-7}
    
    DPVO (+ HMR2.0) \cite{dpvo} & 44.5 & 17.8 & 10.8 & 11.3 & 42.6 & 7.5 \\
    GLAMR \cite{glamr} & 74.9 & 16.7 & 1.8 & 3.2 & 70.6 & 7.4 \\
    TRACE \cite{trace} & 73.4 & 18.8 & 36.2 & 38.0 & 69.6 & 8.8 \\
    
    \cmidrule{1-7}
    \textbf{WHAM (w. DPVO)} & 36.9 & 8.1 & 1.4 & 2.0 & 35.4 & 3.9 \\
    \textbf{WHAM (w. GT gyro)} & \textbf{26.3} & \textbf{7.1} & \textbf{1.4} & \textbf{2.0} & \textbf{23.7} & \textbf{3.5} \\
    \cmidrule{1-7}
    \end{tabular}
    }}}
    \caption{Quantitative comparison of global trajectory estimation on EMDB \cite{emdb} dataset. See text.}
    \label{tab:quant_global}
    \end{table}
\end{center}


==> tables/tableX_quant_global_new_metrics.tex <==
\newcolumntype{?}{!{\vrule width 0.95pt}}

% \begin{center}
    \begin{table}\centering
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.95\columnwidth}{!}{{\small{
    \begin{tabular}{l?cccccc}
    \cmidrule{1-7}
    & \multicolumn{6}{c}{EMDB 2} \\
    \cmidrule(lr){2-7}
    
    Models & WA-MPJPE$_{100}$ & W–MPJPE$_{100}$ & RTE & Jitter & FS & \\
    \cmidrule{1-7}
    
    DPVO (+ HMR2.0) [6, 45] & 662.9 & 2320.9 & 15.8 & 537.4 & 107.6 \\
    GLAMR [54] & 286.2 & 756.1 & 11.4 & 46.2 & 20.7 \\
    TRACE [43] & 544.1 & 2244.9 & 17.7 & 2987.6 & 374.7 \\
    SLAHMR [52] & 807.4 & 336.9 & 10.2 & 31.3 & 14.5 \\
    
    \cmidrule{1-7}
    WHAM w/o traj. ref. & 185.8 & 495.7 & 6.7 & \textbf{19.6} & 7.1 \\
    \textbf{WHAM} & \textbf{165.9} & \textbf{436.4} & \textbf{6.3} & 31.5 & \textbf{5.9} \\
    \cmidrule{1-7}
    \end{tabular}
    }}}
        \vspace{-0.1in}
    \caption{Global motion estimation accuracy on EMDB [15].}
    \label{tab:rebuttal_global}
    \vspace{-0.3em}
    \end{table}

==> tables/tableX_quant_global_v02.tex <==
% \newcolumntype{?}{!{\vrule width 0.95pt}}

% \begin{center}
%     \begin{table}
%     \setlength{\tabcolsep}{3pt}
%     % \renewcommand{\arraystretch}{1.2}
%     \resizebox{0.99\columnwidth}{!}{{\small{
%     \begin{tabular}{l?cccccc}
%     \cmidrule{1-7}
%     & \multicolumn{6}{c}{EMDB Set 2} \\
%     \cmidrule(lr){2-7}
    
%     Models & MPJPE & W-MPJPE & WA-MPJPE & ROE & RTE & ERVE \\
%     \cmidrule{1-7}
    
%     DPVO (+ HMR2.0) \cite{dpvo, hmr2.0} & 47.5 & 2334.0 & 663.3 & 44.5 & 17.8 & 10.8 \\
%     GLAMR \cite{glamr} & 55.9 & 749.4 & 282.4 & 74.9 & 16.7 & 1.8 \\
%     TRACE \cite{trace} & 57.7 & 2227.5 & 543.5 & 73.4 & 18.8 & 36.2 \\
    
%     \cmidrule{1-7}
%     \textbf{WHAM (w. DPVO)} & 41.2 & 447.1 & 169.3 & 36.9 & 8.1 & 1.4 \\
%     \textbf{WHAM (w. GT gyro)} & 41.2 & 437.9 & 166.2 & \textbf{26.3} & \textbf{7.1} & \textbf{1.4} \\
%     \cmidrule{1-7}
%     \end{tabular}
%     }}}
%     \caption{Quantitative comparison of global motion estimation on EMDB \cite{emdb} dataset. See text.}
%     \label{tab:quant_global}
%     \end{table}
% \end{center}


\newcolumntype{?}{!{\vrule width 0.95pt}}

% \begin{center}
    \begin{table}
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.95\columnwidth}{!}{{\small{
    \begin{tabular}{l?cccccc}
    \cmidrule{1-7}
    & \multicolumn{6}{c}{EMDB 2} \\
    \cmidrule(lr){2-7}
    
    Models & PA–MPJPE & W-MPJPE$_{100}$ & WA-MPJPE$_{100}$ & RTE & ROE & ERVE \\
    \cmidrule{1-7}
    
    % DPVO (+ HMR2.0) \cite{dpvo, hmr2.0} & 49.6 & 2320.9 & 662.9 & 17.4 & 43.0 & 112.8 \\
    % GLAMR \cite{glamr} & 56.0 & 756.1 & 286.2 & 16.3 & 72.5 & 18.0 \\
    % TRACE \cite{trace} & 58.0 & 2244.9 & 544.1 & 18.9 & 73.3 & 370.7 \\
    % SLAHMR \cite{slahmr} & 61.5 & 807.4 & 336.9 & 13.7 & 68.7 & 19.7 \\
    % \cmidrule{1-7}
    % \textbf{WHAM (w/ DPVO \cite{dpvo})} & \textbf{41.9} & 446.6 & 169.0 & 8.6 & 40.2 & 14.8 \\
    % \textbf{WHAM (w/ DROID \cite{droid})} & \textbf{41.9} & 439.2 & 166.1 & 7.9 & 35.0 & \textbf{14.7} \\
    % \textbf{WHAM (w/ GT gyro)} & \textbf{41.9} & \textbf{436.4} & \textbf{165.9} & \textbf{6.8} & \textbf{25.8} & 14.8 \\

    DPVO (+ HMR2.0) \cite{dpvo, hmr2.0} & 49.6 & 2320.9 & 662.9 & 17.5 & 44.4 & 112.8 \\
    GLAMR \cite{glamr} & 56.0 & 756.1 & 286.2 & 16.7 & 74.9 & 18.0 \\
    TRACE \cite{trace} & 58.0 & 2244.9 & 544.1 & 18.9 & 72.7 & 370.7 \\
    SLAHMR \cite{slahmr} & 61.5 & 807.4 & 336.9 & 13.8 & 67.9 & 19.7 \\
    \cmidrule{1-7}
    \textbf{WHAM (w/ DPVO \cite{dpvo})} & \textbf{41.9} & 446.6 & 169.0 & 8.8 & 40.4 & 14.8 \\
    \textbf{WHAM (w/ DROID \cite{droid})} & \textbf{41.9} & 439.2 & 166.1 & 8.4 & 36.0 & \textbf{14.7} \\
    \textbf{WHAM (w/ GT gyro)} & \textbf{41.9} & \textbf{436.4} & \textbf{165.9} & \textbf{7.1} & \textbf{26.3} & 14.8 \\
    \cmidrule{1-7}
    \end{tabular}
    }}}
        \vspace{-0.075in}
    \caption{Global motion estimation accuracy on EMDB \cite{emdb}.}
    \label{tab:quant_global}
    \end{table}
% \end{center}



% \newcolumntype{?}{!{\vrule width 0.95pt}}

% \begin{center}
%     \begin{table}
%     \setlength{\tabcolsep}{3pt}
%     % \renewcommand{\arraystretch}{1.2}
%     \resizebox{0.95\columnwidth}{!}{{\small{
%     \begin{tabular}{l?cccccc}
%     \cmidrule{1-7}
%     & \multicolumn{6}{c}{EMDB Set 2} \\
%     \cmidrule(lr){2-7}
    
%     Models & MPJPE & W-MPJPE & WA-MPJPE & RTE & ROE & ERVE \\
%     \cmidrule{1-7}
    
%     DPVO (+ HMR2.0) \cite{dpvo, hmr2.0} & 47.5 & 2334.0 & 663.3 & 17.5 & 43.8 & 112.7 \\
%     GLAMR \cite{glamr} & 55.9 & 749.4 & 282.4 & 16.6 & 73.1 & 18.0 \\
%     TRACE \cite{trace} & 57.7 & 2227.5 & 543.5 & 19.0 & 73.2 & 370.7 \\
%     SLAHMR \cite{slahmr} & & & & & & \\
%     \cmidrule{1-7}
%     \textbf{WHAM (w. DPVO)} & \textbf{41.2} & 447.1 & 169.3 & 8.9 & 40.9 & \textbf{14.8} \\
%     \textbf{WHAM (w. GT gyro)} & \textbf{41.2} & \textbf{437.9} & \textbf{166.2} & \textbf{7.0} & \textbf{26.9} & \textbf{14.8} \\
%     \cmidrule{1-7}
%     \end{tabular}
%     }}}
%     \caption{Quantitative comparison of global motion estimation on EMDB \cite{emdb} dataset. See text.}
%     \label{tab:quant_global}
%     \end{table}
% \end{center}


==> tables/tableX_quant_w_new_accel.tex <==
\newcolumntype{?}{!{\vrule width 0.75pt}}

\begin{table*}[tbh]
\centering
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.8\textwidth}{!}
{\small{
\begin{tabular}{cl?cccc?cccc?cccc}
\cmidrule[0.75pt]{1-14}
& & \multicolumn{4}{c}{3DPW (14)} & \multicolumn{4}{c}{RICH (24)} & \multicolumn{4}{c}{EMDB (24)} \\
% \cmidrule(lr){3-13}
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}

& Models & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} & \scriptsize{PA-MPJPE} & \scriptsize{MPJPE} & \scriptsize{PVE} & \scriptsize{Accel} \\
\cmidrule{1-14}

\multirow{6}{1em}{\rotatebox[origin=c]{90}{per-frame}} 
& SPIN \cite{spin} & 59.2 & 96.9 & 116.4 & 31.4 & 69.7 & 122.9 & 144.2 & 35.2 & 87.1 & 140.3 & 174.9 & 41.3 \\

& PARE$^*$ \cite{pare} & 46.5 & 74.5 & 88.6 & -- & 60.7 & 109.2 & 123.5 & -- & 72.2 & 113.9 & 133.2 & -- \\

& CLIFF$^*$ \cite{cliff} & 43.0 & 69.0 & 81.2 & 22.5 & 56.6 & 102.6 & 115.0 & 22.4 & 68.1 & 103.3 & 128.0 & 24.5 \\

& HybrIK$^*$ \cite{hybrik} & 41.8 & 71.6 &  82.3 & -- & 56.4 & 96.8 & 110.4 & -- & 65.6 & 103.0 & 122.2 & -- \\

& HMR2.0 \cite{hmr2.0} & 44.4 & 69.8 & 84.0 & 18.1 & 48.1 & 96.0 & 110.9 & 18.8 & 60.6 & 98.0 & 120.3 & 19.8 \\

& BEDLAM-CLIFF$^*$ \cite{bedlam} & 43.0 & 66.9 & 78.5 & 31.0 & 50.2 & 84.4 & 95.6 & 29.3 & 60.6 & 98.0 & 111.6 & 36.1 \\
\cmidrule{1-14}

\multirow{12}{1em}{\rotatebox[origin=c]{90}{temporal}} 
& PACE \cite{pace} & -- & -- & -- & -- & 49.3 & --  & -- & 8.8 & -- & -- & -- & -- \\

& TCMR$^*$ \cite{tcmr} & 52.7 & 86.5 & 102.9 & 6.0 & 65.6 & 119.1 & 137.7 &  \textbf{5.0} & 79.6 & 127.6 & 147.9 & \textbf{5.3} \\

& VIBE$^*$ \cite{vibe} & 51.9 & 82.9 & 99.1 & 18.5 & 68.4 & 120.5 & 140.2 & 21.8 & 81.4 & 125.9 & 146.8 & 26.6 \\

& MPS-Net$^*$ \cite{mpsnet}  & 52.1 & 84.3 & 99.7 & 6.5 & 67.1 & 118.2 & 136.7 & 5.8 & 81.3 & 123.1 & 138.4 & 6.2 \\

& GLoT$^*$ \cite{glot} & 50.6 & 80.7 & 96.3 & \textbf{6.0} & 65.6 & 114.3 & 132.7 & 5.2 & 78.8 & 119.7 & 138.4 & 5.4 \\

& GLAMR \cite{glamr} & 51.1 & -- & -- & 8.0 & 79.9 & -- & -- & 107.7 & 73.5 & 113.6 & 133.4 & 32.9 \\

& TRACE$^*$ \cite{trace} & 50.9 & 79.1 & 97.3 & 28.6 & -- & -- & -- & -- & 70.9 & 109.9 & 127.4 & 25.5 \\

& SLAHMR \cite{slahmr} & 55.9& -- & -- & -- & 52.5 & -- & -- & 9.4 & 69.5 & 93.5 & 110.7 & 7.1 \\

% & MAED$^*$ \cite{maed} & 45.7 & 79.1 & 92.6 & 17.6 & -- & -- & -- & & -- & -- & -- & -- \\

\cmidrule{2-14}
& \textbf{WHAM (Res)}$^*$  & 41.7 & 65.7 & 79.8 & 6.6 & 53.1 & 91.4 & 105.6 & 5.3 & 58.9 & 90.3 & 105.7 & 5.7 \\
& \textbf{WHAM (HR)}$^*$  & 40.9 & 64.5 & 78.8 & 6.8 & 50.7 & 88.0 & 100.8 & 5.7 & 56.8 & 88.8 & 105.7 & 6.5 \\
&\textbf{WHAM (ViT)}$^*$ & 37.8 & 60.8 & 73.8 & 6.8 & 46.2 & 84.1 & 95.5 & 5.5 & 52.2 & 85.5 & 101.0 & 5.7 \\
&\textbf{WHAM-B (ViT)}$^*$ & \textbf{37.3} & \textbf{59.2} & \textbf{71.7} & 6.9 & \textbf{44.7} & \textbf{82.6} & \textbf{93.2} & 5.6 & \textbf{49.4} & \textbf{81.5} & \textbf{93.7} & 5.9 \\

\cmidrule[0.75pt]{1-14}
\end{tabular}
}}
    \vspace{-0.075in}
\caption{Quantitative comparison of state-of-the-art models on the 3DPW \cite{3dpw}, RICH \cite{rich}, and EMDB \cite{emdb} datasets. 
Ordering of per-frame and temporal methods is done separately by descending MPJPE on EMDB. For testing on EMDB, we follow the protocol of \textit{EMDB 1} \cite{emdb}. Parenthesis denotes the number of body joints used to compute MPJPE and PA-MPJPE, and $^*$ denotes models trained with the 3DPW training set.
Bold numbers denote the most accurate method in each column. Accel is in $m/\textrm{frame}^2$, all others are in $mm$.
}
\label{tab:quant_hps}
\end{table*}

==> tables/tableX_quant_w_refit.tex <==
\newcolumntype{?}{!{\vrule width 0.95pt}}

\begin{table}\centering
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.8\columnwidth}{!}{{\small{
    \begin{tabular}{l?ccccc}
    \cmidrule{1-5}
    & \multicolumn{4}{c}{3DPW} \\
    \cmidrule(lr){2-5}
    
    Models & PA-MPJPE & MPJPE & PVE & Accel \\
    \cmidrule{1-5}
    
    ReFit & 40.5 & 65.3 & 75.1 & 18.5 \\
    ReFit-B & 38.2 & 57.6 & \textbf{67.6} & 21.4 \\
    
    \cmidrule{1-5}
    \textbf{WHAM (ViT)} & 37.8 & 60.8 & 73.8 & \textbf{6.8} \\
    \textbf{WHAM-B (ViT)} & \textbf{36.1} & \textbf{57.0} & 68.6 & 6.8 \\
    \cmidrule{1-5}
    \end{tabular}
    }}}
    \vspace{-0.1in}
    \caption{Comparison with ReFit on 3DPW [47].}
    \label{tab:rebuttal_refit}
    \vspace{-1.3em}
\end{table}


% % % With "flip_test"
% \begin{table}
%     \setlength{\tabcolsep}{3pt}
%     \resizebox{\columnwidth}{!}{{\small{
%     \begin{tabular}{l?ccccc}
%     \cmidrule{1-5}
%     & \multicolumn{4}{c}{3DPW} \\
%     \cmidrule(lr){2-5}
    
%     Models & PA-MPJPE & MPJPE & PVE & Accel \\
%     \cmidrule{1-5}
    
%     ReFit & 41.2 & 66.0 & 75.8 & 21.7 \\
%     ReFit (w/ flip test) & 40.5 & 65.3 & 75.1 & 18.5 \\
%     ReFit-B & 39.9 & 59.5 & 69.7 & 25.2 \\
%     ReFit-B (w/ flip test) & 38.2 & 57.6 & 67.6 & 21.4 \\
    
%     \cmidrule{1-5}
%     \textbf{WHAM (ViT)} & 37.8 & 60.8 & 73.8 & 6.8 \\
%     \textbf{WHAM (ViT, w/ flip test)} & 36.8 & 60.0 & 71.3 & 6.6 \\
%     \textbf{WHAM-B (ViT)} & 36.8 & 57.8 & 69.6 & 7.0 \\
%     \textbf{WHAM-B (ViT, w/ flip test)} & 36.1 & 57.0 & 68.6 & 6.9 \\
%     \cmidrule{1-5}
%     \end{tabular}
%     }}}
%     \vspace{-0.075in}
%     \caption{Comparison with ReFit on 3DPW [47].}
%     \label{tab:rebuttal_refit}
%     \vspace{-1em}
% \end{table}

==> tables/tableX_rebuttal_ablation.tex <==
\newcolumntype{?}{!{\vrule width 0.95pt}}

% \begin{center}
    \begin{table}
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.2}
    \resizebox{0.95\columnwidth}{!}{{\small{
    \begin{tabular}{l?cccccc}
    \cmidrule{1-7}
    & \multicolumn{6}{c}{EMDB 2} \\
    \cmidrule(lr){2-7}
    
    Models & WA-MPJPE & W–MPJPE & RTE & Jitter & FS & \\
    \cmidrule{1-7}
    w/o traj. ref. & 174.6 & 470.1 & 6.7 & 19.6 & 7.1 \\
    \textbf{WHAM} & 154.6 & 413.8 & 6.3 & 31.5 & 5.9 \\
    \cmidrule{1-7}
    \end{tabular}
    }}}
        \vspace{-0.075in}
    \caption{Ablation study with trajectory refinement unit.}
    \label{tab:rebuttal_contact}
    \end{table}

==> templates/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> templates/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\usepackage{authblk}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


